xCOMET-lite: Bridging the Gap Between Efficiency and Quality in Learned MT Evaluation Metrics

State-of-the-art trainable machine translation evaluation metrics like xCOMET achieve high correlation with human judgment but rely on large encoders (up to 10.7B parameters), making them computationally expensive and inaccessible to researchers with limited resources. To address this issue, we investigate whether the knowledge stored in these large encoders can be compressed while maintaining quality. We employ distillation, quantization, and pruning techniques to create efficient xCOMET alternatives and introduce a novel data collection pipeline for efficient black-box distillation. Our experiments show that, using quantization, xCOMET can be compressed up to three times with no quality degradation. Additionally, through distillation, we create an 278M-sized xCOMET-lite metric, which has only 2.6% of xCOMET-XXL parameters, but retains 92.1% of its quality. Besides, it surpasses strong small-scale metrics like COMET-22 and BLEURT-20 on the WMT22 metrics challenge dataset by 6.4%, despite using 50% fewer parameters. All code, dataset, and models are available online at https://github.com/NL2G/xCOMET-lite.

==> misc/0X-smoothquant.tex <==
% SmoothQuant \cite{DBLP:conf/icml/XiaoLSWDH23} is a PTQ approach leveraging both weights and activations in quantization process. While weight distribution is quite uniform and flat, which is easy to quantize, the scale of outliers in activations is $\sim$100$\times$ larger than most of the activation values which leads to large calculation errors in non-outlier activation channels. To mitigate this problem, it is supposed to migrate the quantization difficulty from activations to weights by simple linear transformation, e.g. in a linear layer:
% $$
% Y = \left(X\diag(s)^{-1}\right)\left(\diag(s)W\right)=\hat{X}\hat{W},
% $$
% where $s\in\mathbb{R}^{C_i}$ is a per-channel smoothing factor.

% To control a tradeoff between computation stability for weights and activations, migration strength $\alpha$ is introduced:
% $$
% s_j = \max\left(|X_j|^{\alpha}\right) / \max\left(|W_j|^{1-\alpha}\right)
% $$

% This approach can also be used for transformer blocks, not only linear activation transformations, but also batch matrix multiplications in attention computation. The huge benefit of this approach is that one can use fast INT8 GEMM CUDA kernels reducing inference time consumption.
